G2T-LLM: Graph-to-Tree Text Encoding for Molecule Generation with Fine-Tuned Large Language Models

We introduce G2T-LLM, a novel approach for molecule generation that uses graph-to-tree text encoding to transform graph-based molecular structures into a hierarchical text format optimized for large language models (LLMs). This encoding converts complex molecular graphs into tree-structured formats, such as JSON and XML, which LLMs are particularly adept at processing due to their extensive pre-training on these types of data. By leveraging the flexibility of LLMs, our approach allows for intuitive interaction using natural language prompts, providing a more accessible interface for molecular design. Through supervised fine-tuning, G2T-LLM generates valid and coherent chemical structures, addressing common challenges like invalid outputs seen in traditional graph-based methods. While LLMs are computationally intensive, they offer superior generalization and adaptability, enabling the generation of diverse molecular structures with minimal task-specific customization. The proposed approach achieved comparable performances with state-of-the-art methods on various benchmark molecular generation datasets, demonstrating its potential as a flexible and innovative tool for AI-driven molecular design.

==> content/visualization_bk.tex <==
\begin{figure*}[t]
    \centering
    \scriptsize
    \begin{tabularx}{\textwidth}{c| c| c| c | c|c| c| c | c| c}
        \hline
        QM9 Ref. & Ours & Grum & GDSS & GDSS-seq 
        & GraphAF & MoFlow & GraphDF & EDP-GNN & GraphEMB \\
        \hline
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/reference/molecule_0.pdf}} &
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/ours/molecule_0.pdf}} &
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/grum/molecule_0.pdf}}&
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/11.png}} &
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/12.png}} &
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/13.png}} &
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/14.png}}&
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/15.png}}&
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/16.png}}&
        \multicolumn{1}{X}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/17.png}} \\
        % \hline
        similarity & 0.5714 & 0.5 & 0.6000 & 
        0.4800 & 0.4800 & 0.3438 
        & 0.2727 & 0.4483 & 0.3182 \\
        \hline
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/reference/molecule_1.pdf}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/ours/molecule_1.pdf}} &
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/grum/molecule_1.pdf}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/21.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/22.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/23.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/24.png}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/25.png}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/26.png}}&
        \multicolumn{1}{c}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/27.png}} \\
        % \hline
        similarity & 0.4516 & 0.4 & 0.4242 & 
        0.3125 & 0.2750 & 0.3514
        & 0.1667 & 0.3529 & 0.2857 \\
        \hline
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/reference/molecule_2.pdf}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/ours/molecule_2.pdf}} &
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/grum/molecule_2.pdf}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/31.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/32.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/33.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/34.png}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/35.png}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/36.png}}&
        \multicolumn{1}{c}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/37.png}} \\
        % \hline
        similarity & 0.3636 & 0.5357 & 0.5357 &
        0.3333 &0.2821 & 0.3529 &
        0.1707 &0.4688 &0.3030 \\
       \hline
       \hline
        Zin250k Ref. & Ours & Grum& GDSS & GDSS-seq 
        & GraphAF & MoFlow & GraphDF & EDP-GNN & GraphEMB \\
        \hline
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/reference/molecule_3.pdf}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/ours/molecule_3.pdf}} &
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/grum/molecule_3.pdf}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/41.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/42.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/43.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/44.png}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/45.png}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/46.png}}&
        \multicolumn{1}{c}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/47.png}} \\
        % \hline
        similarity & 0.3809 & 0.3606 
        &0.3191 &0.2875 &0.2885 &0.2462 &0.2128 &0.2540 &0.2037
 \\
        \hline
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/reference/molecule_4.pdf}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/ours/molecule_4.pdf}} &
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/grum/molecule_4.pdf}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/51.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/52.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/53.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/54.png}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/55.png}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/56.png}}&
        \multicolumn{1}{c}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/57.png}} \\
        % \hline
        similarity & 0.4615 & 0.3275  
        &0.3519 &0.2941 &0.3111 &0.2593 &0.1633 &0.2571 &0.1730 \\
        \hline
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/reference/molecule_5.pdf}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/ours/molecule_5.pdf}} &
        \multicolumn{1}{X|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/grum/molecule_5.pdf}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/61.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/62.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/63.png}} &
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/64.png}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/65.png}}&
        \multicolumn{1}{c|}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/66.png}}&
        \multicolumn{1}{c}{\includegraphics[width=0.08\textwidth]{FIGS/visual/baseline/67.png}} \\
        % \hline
        similarity & 0.4038 & 0.3859
        &0.3871 &0.3559 &0.3800 
        &0.2143 &0.1786 &0.3043 &0.1667\\
        \hline
    \end{tabularx}
    \caption{Visualization of generated molecules.}
    \label{fig:visu}
\end{figure*}
